Intensionalizing Abstract Meaning Representations: Non-Veridicality and Scope

Abstract Meaning Representation (AMR) is a graphical meaning representation language designed to represent propositional information about argument structure. However, at present it is unable to satisfyingly represent non-veridical intensional contexts, often licensing inappropriate inferences. In this paper, we show how to resolve the problem of non-veridicality without appealing to layered graphs through a mapping from AMRs into Simply-Typed Lambda Calculus (STLC). At least for some cases, this requires the introduction of a new role :content which functions as an intensional operator. The translation proposed is inspired by the formal linguistics literature on the event semantics of attitude reports. Next, we address the interaction of quantifier scope and intensional operators in so-called de re/de dicto ambiguities. We adopt a scope node from the literature and provide an explicit multidimensional semantics utilizing Cooper storage which allows us to derive the de re and de dicto scope readings as well as intermediate scope readings which prove difficult for accounts without a scope node.

==> tex/event-semantics-for-attitudes.tex <==
\section{Event Semantics for Attitude Predicates}\label{sec:event-sem-for-att}

We adopt a variant of Kratzer's Davidsonian event semantics for attitude verbs \cite{kratzer2006decomposing}. This account has undergone a number of refinements \cite{moulton2009natural,Elliott2020}(MORE) and has received a significant amount of empirical support (REFERENCES).
More specifically, we propose a translation of attitude reports in AMR into logical forms in which attitude events are associated with a propositional content.

We increase the AMR inventory of semantic roles with a \texttt{:content} role which identifies the propositional content of an event, provided it is associated with one.
We define the interpretation of this relation as follows.\footnote{Where $cf(S)$ returns the characteristic function of $S$.}

\ex.
\a. $\llbracket\texttt{(x\,/\,P\,:content\,A$_{i}$)}\rrbracket^{s}$\\
$ = \lambda \phi. \exists x. \texttt{P}(x)(s) \, \wedge$
\\ \T $\mathcal{C}(x)(s) = \lambda s'. \llbracket \texttt{A}_{i} \rrbracket^{s'} (\lambda y. \top)$
\\ \T\T $\wedge \, \phi(x)(s) $\smallskip \label{ex:content}
\b. where $\mathcal{C}(x)(s) = $
\\ \hspace*{\fill} $ cf\Bigg( \left\{s' \; \Bigg| \begin{tabular}{c} $s'$ is compatible with \\ the content of $x$ in $s$ \end{tabular} \right\} \Bigg)$

The role \texttt{:content} is interpreted as an intensional operator, shifting the situation parameter on the interpretation function and creating a potentially non-veridical environment depending on the attitude predicate $\texttt{P}$ (e.g., \texttt{believe-01} is non-veridical while \texttt{know-01} is veridical).

There are a number of things to observe about the translation in \ref{ex:content}.
Firstly, the translation of the subgraph \texttt{A}$_i$ is fed the dummy formula inside the lambda expression $\lambda s'. \llbracket \texttt{A}_i \rrbracket^{s'} (\lambda y. \top)$.
This means the LF translation of that subgraph will be closed off (i.e., a truth value).
As a result, the content picked out by $\mathcal{C}(x)(s)$ is (a characteristic function of) a set of situations.

Secondly, note that, if the subgraph \texttt{A}$_i$ in \ref{ex:content} is either a constant or recurrent variable then that proposition will be (the characteristic function of) the set of all worlds (since for any \texttt{c} (or \texttt{x}), $(\lambda x. \top)(\texttt{c}) = \top$).
We believe that no natural language sentence describes such a situation, and therefore any AMR with these properties should be avoided.


